Safer Motion Planning of Steerable Needles via a Shaft-to-Tissue Force Model

Steerable needles are capable of accurately targeting difficult-to-reach clinical sites in the body. By bending around sensitive anatomical structures, steerable needles have the potential to reduce the invasiveness of many medical procedures. However, inserting these needles with curved trajectories increases the risk of tissue damage due to perpendicular forces exerted on the surrounding tissue by the needle's shaft, potentially resulting in lateral shearing through tissue. Such forces can cause significant damage to surrounding tissue, negatively affecting patient outcomes. In this work, we derive a tissue and needle force model based on a Cosserat string formulation, which describes the normal forces and frictional forces along the shaft as a function of the planned needle path, friction model and parameters, and tip piercing force. We propose this new force model and associated cost function as a safer and more clinically relevant metric than those currently used in motion planning for steerable needles. We fit and validate our model through physical needle robot experiments in a gel phantom. We use this force model to define a bottleneck cost function for motion planning and evaluate it against the commonly used path-length cost function in hundreds of randomly generated 3-D environments. Plans generated with our force-based cost show a 62% reduction in the peak modeled tissue force with only a 0.07% increase in length on average compared to using the path-length cost in planning. Additionally, we demonstrate the ability to plan motions with our force-based cost function in a lung tumor biopsy scenario from a segmented computed tomography (CT) scan. By planning motions for the needle that aim to minimize the modeled needle-to-tissue force explicitly, our method plans needle paths that may reduce the risk of significant tissue damage while still reaching desired targets in the body.

==> Makefile <==
TOPLEVEL     := needle-force-cost.tex
TARGET       := $(TOPLEVEL:%.tex=%.pdf)
DIFF_TARGET  := diff.pdf
ZIP_TARGET   := $(TOPLEVEL:%.tex=%.zip)
TARGETS      := $(TARGET)
TARGETS      += $(DIFF_TARGET)
COPY_TARGETS := $(TARGETS:%.pdf=%-copy.pdf)
GREY_TARGETS := $(TARGETS:%.pdf=%-grey.pdf)
ZIP_DIR      := $(basename $(ZIP_TARGET))
MAKEFILES    := Makefile
MAKEFILES    += color_out.mk

DEPFILES     :=
DEPFILES     += $(wildcard inputs/*.tex)
DEPFILES     += $(wildcard inputs/algorithms/*.tex)
DEPFILES     += $(wildcard inputs/figures/*.tex)
DEPFILES     += $(wildcard inputs/tables/*.tex)
DEPFILES     += $(wildcard inputs/notes/*.tex)
DEPFILES     += $(wildcard *.bib)
DEPFILES     += $(wildcard *.bst)
DEPFILES     += $(wildcard *.cls)
DEPFILES     += $(wildcard *.sty)
DEPFILES     += $(wildcard images/*.pdf)
DEPFILES     += $(wildcard images/timing/*.pdf)
DEPFILES     += $(wildcard images/physical-robot/*.pdf)
DEPFILES     += $(wildcard images/physical-robot/*.pdf_tex)
DEPFILES     += $(TOPLEVEL)
DEPFILES     += $(MAKEFILES)

ZIPFILES     :=
ZIPFILES     += $(TOPLEVEL)
ZIPFILES     += $(MAKEFILES)
ZIPFILES     += images/12paths-run02-plot-wide-p30-01-take2.pdf
ZIPFILES     += images/12paths-run02-plot-wide-p30-01-take2.pdf_tex
ZIPFILES     += images/12paths-run02-plot-wide-p39-01-take2.pdf
ZIPFILES     += images/12paths-run02-plot-wide-p39-01-take2.pdf_tex
ZIPFILES     += images/correlation-all-small.pdf
ZIPFILES     += images/correlation-all-small.pdf_tex
ZIPFILES     += images/example-path-forces.pdf
ZIPFILES     += images/example-path-forces.pdf_tex
ZIPFILES     += images/example-path-three.pdf
ZIPFILES     += images/example-path-three.pdf_tex
ZIPFILES     += images/multifit-tau.pdf
ZIPFILES     += images/multifit-tau.pdf_tex
ZIPFILES     += images/needle-path-and-piece-latex.pdf
ZIPFILES     += images/needle-path-and-piece-latex.pdf_tex
ZIPFILES     += images/path-in-anatomy.pdf
ZIPFILES     += images/path-in-anatomy.pdf_tex
ZIPFILES     += images/physical-robot.pdf
ZIPFILES     += images/physical-robot.pdf_tex
ZIPFILES     += images/shearing-p01-01.pdf
ZIPFILES     += images/shearing-p01-01.pdf_tex
ZIPFILES     += images/sphere-path-cost.pdf
ZIPFILES     += images/sphere-path-cost.pdf_tex
ZIPFILES     += images/sphere-path-seed-0393-all.pdf
ZIPFILES     += images/sphere-path-seed-0393-all.pdf_tex
ZIPFILES     += inputs/alg-planner.tex
ZIPFILES     += inputs/fig-correlation.tex
ZIPFILES     += inputs/fig-model-forces-p30.tex
ZIPFILES     += inputs/fig-model-forces.tex
ZIPFILES     += inputs/fig-multifit-tau.tex
ZIPFILES     += inputs/fig-needle-path-and-piece.tex
ZIPFILES     += inputs/fig-needle-path-spheres.tex
ZIPFILES     += inputs/fig-path-in-anatomy.tex
ZIPFILES     += inputs/fig-physical-robot.tex
ZIPFILES     += inputs/fig-shearing.tex
ZIPFILES     += inputs/fig-sphere-path-cost.tex
ZIPFILES     += inputs/fig-three-path-force.tex
ZIPFILES     += inputs/fig-tissue-force-heatmap.tex
ZIPFILES     += inputs/hdr-abstract.tex
ZIPFILES     += inputs/hdr-authors.tex
ZIPFILES     += inputs/hdr-newcommands.tex
ZIPFILES     += inputs/hdr-override-catchline.tex
ZIPFILES     += inputs/hdr-usepackage.tex
ZIPFILES     += inputs/sec-acknowledgment.tex
ZIPFILES     += inputs/sec-conclusion.tex
ZIPFILES     += inputs/sec-experiment.tex
ZIPFILES     += inputs/sec-intro.tex
ZIPFILES     += inputs/sec-method.tex
ZIPFILES     += inputs/sec-related-work.tex
ZIPFILES     += inputs/tbl-models.tex
ZIPFILES     += references.bib
ZIPFILES     += ws-jmrr.bst
ZIPFILES     += ws-jmrr.cls
ZIPFILES     += ws-rotating.sty

GARBAGE      :=
GARBAGE      += comment.cut
GARBAGE      += $(TOPLEVEL:%.tex=%.log)
GARBAGE      += $(TOPLEVEL:%.tex=%.out)
GARBAGE      += $(TOPLEVEL:%.tex=%.aux)
GARBAGE      += $(TOPLEVEL:%.tex=%.dvi)
GARBAGE      += $(TOPLEVEL:%.tex=%.cb)
GARBAGE      += $(TOPLEVEL:%.tex=%.cb2)
GARBAGE      += $(TOPLEVEL:%.tex=%.bbl)
GARBAGE      += $(TOPLEVEL:%.tex=%.blg)
GARBAGE      += $(TOPLEVEL:%.tex=%.tdo)
GARBAGE      += $(TOPLEVEL:%.tex=%.markdown.in)
GARBAGE      += $(TOPLEVEL:%.tex=%.markdown.lua)
GARBAGE      += $(TOPLEVEL:%.tex=%.markdown.out)
GARBAGE      += $(TOPLEVEL:%.tex=%.fdb_latexmk)
GARBAGE      += $(TOPLEVEL:%.tex=%.fls)
GARBAGE      += $(addprefix _markdown_,$(TOPLEVEL:%.tex=%))
GARBAGE      += $(addprefix _minted-,$(TOPLEVEL:%.tex=%))
GARBAGE      += $(wildcard figures/*-eps-converted-to.pdf)

TEXPATH      ?= .:inputs:

# To use custom fonts, build with xelatex instead
#LATEXDIFF    := TEXINPUTS=$(TEXPATH) latexdiff
LATEXDIFF     := latexdiff
# Choose latexdiff type (only uncomment one of them)
LATEXDIFF     += -t UNDERLINE     # (default) added text is wavy-underlined and blue, discarded text is struck out and red;
#LATEXDIFF     += -t CTRADITIONAL  # added text is blue and set in sans-serif, and a red footnote is created for each discarded piece of text;
#LATEXDIFF     += -t TRADITIONAL   # like CTRADITIONAL but without the use of colour;
#LATEXDIFF     += -t CFONT         # added text is blue and set in sans-serif, and discarded text is red and very small size;
#LATEXDIFF     += -t FONTSTRIKE    # added text is set in sans-serif, discarded text small and struck out;
#LATEXDIFF     += -t CHANGEBAR     # added text is blue, and discarded text is red. Additionally, the changed text is marked with a bar in the margin.
# You may exclude specific text commands
#LATEXDIFF    += --exclude-textcmd="section,subsection"

LATEXPAND     := latexpand

LATEX         := pdflatex
LATEX         += -shell-escape
DETEX         := TEXINPUTS="$(TEXPATH)" detex
DETEX_DEFAULTS := array,eqnarray,equation,longtable,picture,tabular,verbatim

# LATEX_BUILD command: uses latexmk if available, else calls latex, bibtex, latex*2
#   $(call LATEX_BUILD,$*)
ifeq (,$(shell which latexmk))
define LATEX_BUILD
	$(LATEX) $1.tex </dev/null >/dev/null || (tail -n 30 $1.log && false)
	-bibtex $1.tex  </dev/null >/dev/null
	$(LATEX) $1.tex </dev/null >/dev/null
	$(LATEX) $1.tex </dev/null >/dev/null
endef
else
define LATEX_BUILD
	latexmk -pdf -pdflatex="$(LATEX) %O %S" $1.tex </dev/null >/dev/null || (tail -n 30 $1.log && false)
endef
endif

-include color_out.mk

ifndef VERBOSE
.SILENT:
endif

.PHONY: default
default: $(TARGET) copy
copy: $(TARGET:%.pdf=%-copy.pdf)
grey: $(TARGET:%.pdf=%-grey.pdf)

.PHONY: all
all: $(TARGETS) $(COPY_TARGETS) $(GREY_TARGETS) $(ZIP_TARGET)

.PHONY: zip arxiv
zip: $(ZIP_TARGET)
arxiv: zip

$(TARGET): $(MAKEFILES) $(DEPFILES)

# print statistics of a tex file compilation
# @param $1: name of the log file
define TEX_STATS
	echo
	$(call bold_color,BLUE,$1 statistics:)
	echo "    ----"
	if grep "^mylog: mytodo" $1 >/dev/null; then \
	  $(call color_out_noline,RED,  unaddressed todos:      ); \
	else \
	  $(call color_out_noline,BLUE,  unaddressed todos:      ); \
	fi
	grep "^mylog: mytodo" $1 | wc -l
	echo "    ----"
	$(call color_out_noline,BLUE,  overfull:               )
	grep "^Overfull" $1 | wc -l
	$(call color_out_noline,BLUE,  underfull:              )
	grep "^Underfull" $1 | wc -l
	echo "    ----"
	$(call color_out_noline,BLUE,  total warnings:         )
	grep -i warning $1 | wc -l
	$(call color_out_noline,BLUE,  undefined citations:    )
	grep "Warning: Citation .* undefined" $1 | wc -l
	$(call color_out_noline,BLUE,  undefined references:   )
	grep "Warning: Reference .* undefined" $1 | wc -l
	$(call color_out_noline,BLUE,  duplicate labels:       )
	grep "Warning: Label .* multiply defined" $1 | wc -l
	echo "    ----"
	if [ "$$(type -P detex)" ]; then \
		$(call color_out_noline,BLUE,  total word count:       ); \
		$(DETEX) -e $(DETEX_DEFAULTS) $(1:%.log=%.tex) | wc -w; \
		$(call color_out_noline,BLUE,  without fig+tbl+alg:    ); \
		$(DETEX) -e $(DETEX_DEFAULTS),figure,table,algorithm  $(1:%.log=%.tex) | wc -w; \
		$(call color_out_noline,BLUE,  fig+tbl+alg words:      ); \
		echo $$($(DETEX) -e $(DETEX_DEFAULTS) $(1:%.log=%.tex) | wc -w) - $$($(DETEX) -e $(DETEX_DEFAULTS),figure,table,algorithm $(1:%.log=%.tex) | wc -w) | bc; \
	  echo "    ----"; \
	fi
	$(call color_out_noline,BLUE,  pages:                  )
	grep "[0-9]\+ page" $1 | sed -e 's/.*(\([0-9]\+\) page.*/\1/g'
	echo "    ----"
	echo
endef

%.pdf: %.tex $(MAKEFILES)
	@$(call color_out,GREEN,$< -> $@)
	$(call LATEX_BUILD,$*)
	$(call TEX_STATS,$*.log)

%-copy.pdf: %.pdf
	@$(call color_out,GREEN,$< -> $@)
	cp $< $@

%-grey.pdf: %.pdf
	@$(call color_out,GREEN,$< -> $@)
	gs \
	  -sOutputFile="$@" \
	  -sDEVICE=pdfwrite \
	  -sColorConversionStrategy=Gray \
	  -dProcessColorModel=/DeviceGray \
	  -dCompatibilityLevel=1.4 \
	  -dNOPAUSE \
	  -dBATCH \
	  -q \
	  "$<"

images/%.eps: images/%.dot
	@$(call color_out,GREEN,$< -> $@)
	dot $< -Tps -o $@

images/%.ps: images/%.tex
	@$(call color_out,GREEN,$< -> $@)
	(cd images && $(LATEX) $(notdir $<)) </dev/null >/dev/null \
		|| (tail -n 30 $(<:%.tex=%.log) && false)

.PHONY: diff
diff: diff.pdf

diff.tex: old.tex new.tex
	@$(call color_out,GREEN,old.tex + new.tex -> $@)
	$(LATEXDIFF) old.tex new.tex 2>/dev/null > diff.tex

new.tex: $(MAKEFILES) $(DEPFILES)
	@$(call color_out,GREEN,$(TOPLEVEL) -> new.tex)
	TEXINPUTS="$(TEXPATH)" $(LATEXPAND) --fatal --verbose --output new.tex $(TOPLEVEL) 2>/dev/null

.PHONY: count
count: new.tex
	@$(call color_out,GREEN,count from new.tex)
	TEXINPUTS="$(TEXPATH)" texcount -merge new.tex

GARBAGE    += new.tex
GARBAGE    += diff.tex
TARGETS    += diff.pdf
GARBAGE    += old.log
GARBAGE    += old.out
GARBAGE    += old.aux
GARBAGE    += old.dvi
GARBAGE    += old.cb
GARBAGE    += old.cb2
GARBAGE    += old.bbl
GARBAGE    += old.blg
GARBAGE    += old.tdo
GARBAGE    += old.markdown.in
GARBAGE    += old.markdown.lua
GARBAGE    += old.markdown.out
GARBAGE    += old.pdf
GARBAGE    += new.log
GARBAGE    += new.out
GARBAGE    += new.aux
GARBAGE    += new.dvi
GARBAGE    += new.cb
GARBAGE    += new.cb2
GARBAGE    += new.bbl
GARBAGE    += new.blg
GARBAGE    += new.tdo
GARBAGE    += new.markdown.in
GARBAGE    += new.markdown.lua
GARBAGE    += new.markdown.out
GARBAGE    += new.pdf
GARBAGE    += new.tex
GARBAGE    += diff.log
GARBAGE    += diff.out
GARBAGE    += diff.aux
GARBAGE    += diff.dvi
GARBAGE    += diff.cb
GARBAGE    += diff.cb2
GARBAGE    += diff.bbl
GARBAGE    += diff.blg
GARBAGE    += diff.tdo
GARBAGE    += diff.markdown.in
GARBAGE    += diff.markdown.lua
GARBAGE    += diff.markdown.out
GARBAGE    += diff.tex

.PHONY: clean
clean:
	rm -rf $(GARBAGE)

.PHONY: veryclean
veryclean: clean
	rm -f $(TARGETS)
	rm -f $(COPY_TARGETS)
	rm -f $(GREY_TARGETS)
	rm -rf $(ZIP_DIR)
	rm -f $(ZIP_TARGET)

.PHONY: distclean
distclean: veryclean

$(ZIP_DIR):
	@mkdir -p $(ZIP_DIR)

# @param 1: source file
# @param 2: destination directory
define COPY_TO_PATH
	mkdir -p $(strip $2)/$(strip $(dir $1))
	cp $1 $2/$1
	
endef

$(ZIP_TARGET): $(ZIPFILES) | $(ZIP_DIR)
	@echo "copying files into $(ZIP_DIR)/"
	@$(foreach f,$(ZIPFILES),$(call COPY_TO_PATH,$f,$(ZIP_DIR)))
	@echo "$(ZIP_DIR)/* -> $(ZIP_TARGET)"
	@zip -r $(ZIP_TARGET) $(ZIP_DIR) >/dev/null

